Mining Scientific Workflows for Anomalous Data Transfers

Modern scientific workflows are data-driven and are often executed on distributed, heterogeneous, high-performance computing infrastructures. Anomalies and failures in the workflow execution cause loss of scientific productivity and inefficient use of the infrastructure. Hence, detecting, diagnosing, and mitigating these anomalies are immensely important for reliable and performant scientific workflows. Since these workflows rely heavily on high-performance network transfers that require strict QoS constraints, accurately detecting anomalous network performance is crucial to ensure reliable and efficient workflow execution. To address this challenge, we have developed X-FLASH, a network anomaly detection tool for faulty TCP workflow transfers. X-FLASH incorporates novel hyperparameter tuning and data mining approaches for improving the performance of the machine learning algorithms to accurately classify the anomalous TCP packets. X-FLASH leverages XGBoost as an ensemble model and couples XGBoost with a sequential optimizer, FLASH, borrowed from search-based Software Engineering to learn the optimal model parameters. X-FLASH found configurations that outperformed the existing approach up to 28\%, 29\%, and 40\% relatively for F-measure, G-score, and recall in less than 30 evaluations. From (1) large improvement and (2) simple tuning, we recommend future research to have additional tuning study as a new standard, at least in the area of scientific workflow anomaly detection.

==> TuningWorkflow (MSR)/choices.tex <==
\begin{table*}[!t]
\caption{Hyperparameter tuning options explored by DODGE($\epsilon$) in this paper, drawn from recent SE hyperparameter optimization work~\citep{ghotra2015revisiting,fu2016tuning,agrawal2018better,agrawal2018wrong} then consulting the documentation of a widely-used library
(Scikit-learn by~\cite{pedregosa2011scikit}). Randint,  randuniform and randchoice are  all random functions to choose either integer, float, or a choice among the parameter ranges.}\label{tbl:options}
\vspace{-7pt}
% \label{tab:dodge}
%\captionsetup{font=footnotesize}

\footnotesize
 
 \begin{tcolorbox}[colback=white]
 \begin{flushleft}
 \vspace{-5pt}
 {\bf DATA PRE-PROCESSORS:} 
\vspace{-10pt}
\begin{multicols}{2}
\bi
\item StandardScaler
\item MinMaxScaler
 \item KernelCenterer
\item Normalizer(norm=a): a = randchoice([`l1', `l2',`max'])
 \item MaxAbsScaler
 \item Binarizer(threshold=a): a =  randuniform(0,100)
\ei
\end{multicols}
\vspace{-13pt}
\bi
 \item RobustScaler(quantile\_range=(a, b)): a, b =  randint(0,50), randint(51,100) 
 \item QuantileTransformer(n\_quantiles=a,  output\_distribution=c, subsample=b). a, b = randint(100, 1000), randint(1000, 1e5);
   c=randchoice([`normal',`uniform']).
    \item SMOTE(a=n\_neighbors, b=n\_synthetics,  c=Minkowski\_exponent). a,b = randit(1,20),randchoice(50,100,200,400). c = randuniform(0.1,5) 
     
\ei
\rule{\linewidth}{0.4pt}

 \vspace{1pt}
\vspace{5pt}
\textbf{LEARNERS:}  

\noindent
\bi
\item DecisionTreeClassifier(criterion=b, splitter=c, min\_samples\_split=a).
    a, b, c= randuniform(0.0,1.0), randchoice([`gini',`entropy']),   randchoice([`best',`random']).
  
\item RandomForestClassifier(n\_estimators=a,criterion=b,  min\_samples\_split=c).  a,b,c = randint(50, 150), randchoice(['gini', 'entropy']),  randuniform(0.0, 1.0) 
     
\item MultinomialNB(alpha=a): a = randuniform(0.0,0.1)
\item KNeighborsClassifier(n\_neighbors=a, weights=b, p=d, metric=c).  a, b,c  = randint(2, 25), randchoice([`uniform', `distance']),  randchoice([`minkowski',`chebyshev']). 
  If c=='minkowski': d= randint(1,15)  else:  d=2

\ei
\vspace{-5pt}


\end{flushleft}
\end{tcolorbox}
\vspace{-17pt}
\end{table*}

==> TuningWorkflow (MSR)/features.tex <==
\begin{table}[!t]
\footnotesize
\begin{center}
\caption{Top 10\% important TCP Statistics features collected by the Tstat tool identified by the state-of-the-art model of \cite{tcp_indis_19} across the data. (S2C: Server to Client, C2S: Client to Server, Both: C2S and S2C)}
\label{tbl:attributes}
\vspace{-3pt}
\begin{tabular} {c|c|l}
Attribute &  Types &  Description \\ \hline
 c\_bytes\_all & C2S	 & Number of bytes transmitted in the \\
 & & payload, including retransmissions \\ 
 c\_pkts\_retx & C2S & Number of retransmitted segments \\ 
 c\_bytes\_retx & C2S  & Number of retransmitted bytes \\ 
 s\_ack\_cnt\_p & S2C	& Number of segments with ACK field \\
 & & set to 1 and no data \\
 durat & ---	& Flow duration since first to last packet \\
 c/s\_first & Both & Client/Server first segment with payload \\
 & & since the first flow segment \\
 c/s\_last  & Both & Client/Server last segment with payload \\
 & & since the first flow segment \\
 c/s\_first\_ack & Both & Client/Server first ACK segment (without  \\
  & & SYN) since the first flow segment	 \\
 c/s\_rtt\_avg & Both & Average RTT computed measuring the time \\
 & & elapsed between the data segment and \\
 & & the corresponding ACK\\
c/s\_rtt\_min & Both & Minimum RTT observed in connection lifetime \\
c/s\_rtt\_max & Both & Maximum RTT observed in connection lifetime \\
%  s\_rtt\_std & S2C & Standard deviation of the RTT \\
%  c\_cwin\_max & C2S & Maximum in-flight-size computed as the difference between the largest sequence number \\
%  & & so far, and the corresponding last ACK message on the reverse path. It is an estimate\\
%  & &  of the congestion window \\
%  c\_pkts\_reor & C2S & Number of packet reordering observed \\
%  c\_pkts\_dup & C2S & Number of network duplicates observed
% \\
%  c\_pkts\_unk & C2S  & Number of segments not in sequence or duplicate which are not classified as specific events\\
%  s\_sack\_cnt &  S2C & Number of SACK messages sent \\
%  s\_win\_max &  S2C & Maximum segment size observed \\
%  c\_pkts\_push & C2S & Number of push separated messages from Client to Server\\
%  c/s\_last\_handshakeT & Both & For Transport Layer Security (TLS) flows, time of Client/Server last packet seen before 
%  \\& &  first Application Data (relative)
% \\
%  c\_appdataT & C2S & For TLS flows, time between the Client first Application Data message and the first \\ & &    flow segment \\
 \hline
 
% ['c_port:2', 'c_bytes_all:9', 'c_pkts_retx:10', 'c_bytes_retx:11', 'c_pkts_ooo:12', 's_port:16', 's_ack_cnt_p:20', 'durat:31', 'c_first:32', 's_first:33', 'c_last:34', 'c_last:35', 'c_first_ack:36', 's_first_ack:37', 'c_rtt_avg:45', 'c_rtt_min:46', 'c_rtt_max:47', 'c_rtt_std:48', 'c_rtt_cnt:49', 's_rtt_avg:52', 's_rtt_min:53', 's_rtt_max:54', 's_rtt_std:55', 'c_cwin_max:76', 'c_pkts_reor:81', 'c_pkts_dup:82', 'c_pkts_unk:83', 's_sack_cnt:92', 's_win_max:96', 'c_pkts_push:114', 'c_last_handshakeT:121', 's_last_handshakeT:122', 'c_appdataT:123']
\end{tabular}
\end{center}
\vspace{-15pt}
%\end{table}
\end{table}

==> TuningWorkflow (MSR)/name.tex <==
1/ need to explain why use these data miners
2/ need to add dodge 
3/ 271 and 273 is it better for background knowledge.
4/ 460, the DODGE list
5/ Describe gaussian process model, FLASH beat GP model and DODGE beats GA and DE. Mentioned other people work before using DODGE and FLASH. 
6/ Describe FLASH as DODGE list to be the same formatting. 
7/ Correct the mismatched name of the stats testing
8/ 3 charts for figure with dataset names

==> TuningWorkflow (MSR)/records.tex <==
\begin{table*}[!htp]
\scriptsize
\caption{Recall, F-measure, and G-score (higher the better) results are reported between all the methods that are ranked by Scott-Knott statistical tests. Medians and IQRs (delta between 75th percentile and 25th percentile, lower the better) are calculated for easy comparisons. The best performing one is noted as a gray cell for each metric per column. The column \textbf{\#Best} shows the number of projects each treatment performs the best in.}
\centering
\setlength\tabcolsep{4pt}
\begin{tabular}{p{.065\linewidth}|p{.1\linewidth}|c|c|c|c|c|c|c|c|c|c|c}
\multirow{2}{*}{\textbf{Metrics}}   & \multirow{2}{*}{\textbf{Treatment}}   & \multicolumn{4}{c|}{\textbf{Mice and Elephant Flows}} & \multicolumn{4}{c|}{\textbf{1000 Genome Workflow}} & \multirow{2}{*}{\textbf{Median}} & \multirow{2}{*}{\textbf{IQR}} & \multirow{2}{*}{\textbf{\#BEST}} \\
\cline{3-10}
&  & \textbf{HAMILTON}	&	\textbf{BBR}	&	\textbf{RENO}	&	\textbf{CUBIC}	&	\textbf{HAMILTON}	&	\textbf{BBR}	&	\textbf{RENO}	&	\textbf{CUBIC} & & & 
\\\hline
% \multirow{7}{*}{Accuracy} &
% X-FLASH	&	\cellcolor{gray!20} 85	&	\cellcolor{gray!20}56	&	\cellcolor{gray!20}91	&	\cellcolor{gray!20}77	&	\cellcolor{gray!20}92	&	\cellcolor{gray!20}93	&	\cellcolor{gray!20}91	&	\cellcolor{gray!20}96	&	91	&	9 & 8\\
% & FLASH\_CART	&	83	&	53	&	87	&	73	&	82	&	82	&	83	&	90	&	83	&	4 & 0\\
% & FLASH\_RF	&	82	&	\cellcolor{gray!20}55	&	87	&	74	&	89	&	87	&	86	&	94	&	87	&	7 & 1\\
% & DODGE	&	79	&	53	&	87	&	73	&	82	&	83	&	81	&	89	&	82	&	6 & 0\\
% & CART	&	83	&	\cellcolor{gray!20}54	&	87	&	74	&	84	&	84	&	84	&	90	&	84	&	4 & 1 \\
% & RF	&	82	&	\cellcolor{gray!20}55	&	87	&	74	&	89	&	88	&	85	&	94	&	86	&	8 & 1\\
% & XGBOOST	&	75	&	49	&	81	&	69	&	85	&	85	&	82	&	92	&	82	&	11 & 0\\
% \hline
% \multirow{7}{*}{Precision} &
% X-FLASH	&	\cellcolor{gray!20}83	&	\cellcolor{gray!20}52	&	\cellcolor{gray!20}88	&	65	&	\cellcolor{gray!20}87	&	\cellcolor{gray!20}91	&	\cellcolor{gray!20}89	&	\cellcolor{gray!20}96	&	88	&	11 & 7\\
% & FLASH\_CART	&	78	&	\cellcolor{gray!20}44	&	85	&	65	&	70	&	80	&	46	&	86	&	74	&	21 & 1\\
% & FLASH\_RF	&	78	&	\cellcolor{gray!20}52	&	84	&	\cellcolor{gray!20}69	&	84	&	85	&	\cellcolor{gray!20}88	&	93	&	84	&	10 & 3\\
% & DODGE	&	76	&	\cellcolor{gray!20}50	&	85	&	\cellcolor{gray!20}68	&	71	&	80	&	66	&	87	&	74	&	13 & 2\\
% & CART	&	80	&	\cellcolor{gray!20}51	&	85	&	\cellcolor{gray!20}68	&	72	&	82	&	67	&	87	&	76	&	15 & 2\\
% & RF	&	78	&	\cellcolor{gray!20}51	&	84	&	\cellcolor{gray!20}69	&	83	&	86	&	\cellcolor{gray!20}87	&	94	&	84	&	10 & 3\\
% & XGBOOST	&	74	&	\cellcolor{gray!20}52	&	77	&	62	&	78	&	83	&	82	&	91	&	78	&	11 & 1\\
% \hline
\multirow{7}{*}{Recall} &
X-FLASH	&	\cellcolor{gray!20}84	&	\cellcolor{gray!20}50	&	\cellcolor{gray!20}89	&	\cellcolor{gray!20}70	&	\cellcolor{gray!20}85	&	\cellcolor{gray!20}92	&	\cellcolor{gray!20}73	&	\cellcolor{gray!20}95	&	85	&	17 & 8\\
& FLASH\_CART	&	81	&	\cellcolor{gray!20}49	&	84	&	\cellcolor{gray!20}68	&	71	&	82	&	66	&	87	&	76	&	15 & 2\\
& FLASH\_RF	&	80	&	\cellcolor{gray!20}49	&	84	&	\cellcolor{gray!20}68	&	78	&	85	&	52	&	91	&	79	&	20 & 2\\
& DODGE	&	78	&	48	&	85	&	\cellcolor{gray!20}68	&	70	&	81	&	63	&	86	&	74	&	15 & 1\\
& CART	&	81	&	\cellcolor{gray!20}49	&	84	&	\cellcolor{gray!20}68	&	72	&	82	&	67	&	87	&	77	&	14 &		2\\
& RF	&	80	&	\cellcolor{gray!20}49	&	84	&	\cellcolor{gray!20}68	&	77	&	85	&	52	&	91	&	79	&	20 &	2\\
& XGBOOST	&	71	&	39	&	74	&	58	&	69	&	81	&	39	&	89	&	70	&	22 &	0\\
\hline
\multirow{7}{*}{F-measure} &
X-FLASH	&	\cellcolor{gray!20}83	&	\cellcolor{gray!20}49	&	\cellcolor{gray!20}88	&	\cellcolor{gray!20}71	&	\cellcolor{gray!20}86	&	\cellcolor{gray!20}91	&	\cellcolor{gray!20}80	&	\cellcolor{gray!20}94	&	85	&	11 &	8\\
& FLASH\_CART	&	81	&	\cellcolor{gray!20}48	&	85	&	\cellcolor{gray!20}69	&	70	&	80	&	67	&	87	&	75	&	13 &	2\\
& FLASH\_RF	&	79	&	\cellcolor{gray!20}49	&	84	&	\cellcolor{gray!20}69	&	80	&	85	&	62	&	92	&	80	&	17 &	2\\
& DODGE	&	77	&	\cellcolor{gray!20}48	&	85	&	\cellcolor{gray!20}68	&	70	&	80	&	63	&	85	&	74	&	14 &	2\\
& CART	&	81	&	\cellcolor{gray!20}49	&	84	&	\cellcolor{gray!20}69	&	73	&	82	&	67	&	86	&	77	&	14 &	2\\
& RF	&	79	&	\cellcolor{gray!20}49	&	84	&	\cellcolor{gray!20}69	&	81	&	85	&	62	&	91	&	80	&	17 &	2\\
& XGBOOST	&	72	&	36	&	75	&	56	&	73	&	82	&	45	&	90	&	73	&	23 &	0\\
\hline
\multirow{7}{*}{G-score} &
X-FLASH	&	\cellcolor{gray!20}88	&	\cellcolor{gray!20}62	&	\cellcolor{gray!20}92	&	\cellcolor{gray!20}80	&	\cellcolor{gray!20}90	&	\cellcolor{gray!20}94	&	\cellcolor{gray!20}83	&	\cellcolor{gray!20}96	&	89	&	10 &	8\\
& FLASH\_CART	&	86	&	\cellcolor{gray!20}62	&	89	&	\cellcolor{gray!20}78	&	78	&	87	&	78	&	91	&	82	&	9 &	2\\
& FLASH\_RF	&	86	&	\cellcolor{gray!20}62	&	89	&	\cellcolor{gray!20}78	&	85	&	89	&	64	&	94	&	86	&	14 &	2\\
& DODGE	&	85	&	61	&	90	&	\cellcolor{gray!20}78	&	79	&	87	&	73	&	91	&	82	&	11 &	1\\
& CART	&	87	&	\cellcolor{gray!20}62	&	90	&	\cellcolor{gray!20}78	&	81	&	87	&	77	&	91	&	84	&	10 &	2\\
& RF	&	86	&	\cellcolor{gray!20}62	&	89	&	\cellcolor{gray!20}78	&	85	&	90	&	65	&	94	&	86	&	14 &	2 \\
& XGBOOST	&	80	&	52	&	83	&	70	&	79	&	88	&	52	&	93	&	80	&	18 &	0
\\


\hline
\end{tabular}
\vspace{-10pt}
\label{tbl:rq1}
\end{table*}

==> name.tex <==
1/ need to explain why use these data miners
2/ need to add dodge 
3/ 271 and 273 is it better for background knowledge.
4/ 460, the DODGE list
5/ Describe gaussian process model, FLASH beat GP model and DODGE beats GA and DE. Mentioned other people work before using DODGE and FLASH. 
6/ Describe FLASH as DODGE list to be the same formatting. 
7/ Correct the mismatched name of the stats testing
8/ 3 charts for figure with dataset names
